Do LLM Agents Have Regret? A Case Study in Online Learning and Games

Large language models (LLMs) have been increasingly employed for (interactive) decision-making, via the development of LLM-based autonomous agents. Despite their emerging successes, the performance of LLM agents in decision-making has not been fully investigated through quantitative metrics, especially in the multi-agent setting when they interact with each other, a typical scenario in real-world LLM-agent applications. To better understand the limits of LLM agents in these interactive environments, we propose to study their interactions in benchmark decision-making settings in online learning and game theory, through the performance metric of \emph{regret}. We first empirically study the {no-regret} behaviors of LLMs in canonical (non-stationary) online learning problems, as well as the emergence of equilibria when LLM agents interact through playing repeated games. We then provide some theoretical insights into the no-regret behaviors of LLM agents, under certain assumptions on the supervised pre-training and the rationality model of human decision-makers who generate the data. Notably, we also identify (simple) cases where advanced LLMs such as GPT-4 fail to be no-regret. To promote the no-regret behaviors, we propose a novel \emph{unsupervised} training loss of \emph{regret-loss}, which, in contrast to the supervised pre-training loss, does not require the labels of (optimal) actions. We then establish the statistical guarantee of generalization bound for regret-loss minimization, followed by the optimization guarantee that minimizing such a loss may automatically lead to known no-regret learning algorithms. Our further experiments demonstrate the effectiveness of our regret-loss, especially in addressing the above ``regrettable'' cases.

==> abstract.tex <==
\begin{abstract}     
\iclr{\safevspace{-10pt}} 
Large language models (LLMs)  have been increasingly employed for (interactive) decision-making, via the development of LLM-based autonomous agents.  Despite their emerging successes, the performance of LLM agents in decision-making has not been fully investigated through quantitative metrics, especially in the multi-agent setting when they interact with each other, a typical scenario in real-world LLM-agent applications. To better understand the limits of LLM agents in these interactive environments, we propose to study their interactions in benchmark decision-making settings in online learning and game theory, through the   performance metric of \emph{regret}. We first empirically study the {no-regret} behaviors of LLMs in canonical (non-stationary) online learning problems, as well as the emergence of equilibria when LLM agents interact through playing repeated games. We then provide some theoretical insights into the no-regret behaviors of LLM agents, under certain assumptions on the supervised pre-training and the rationality model of human decision-makers who generate the data. Notably, we also identify (simple) cases where advanced LLMs such as GPT-4 fail to be no-regret. To promote the no-regret behaviors, we propose a novel \emph{unsupervised} training loss of \emph{regret-loss}, which, in contrast to the supervised pre-training loss, does not require the labels of (optimal) actions. We then establish the statistical guarantee of generalization bound for  regret-loss minimization, followed by the optimization guarantee that minimizing such a loss may automatically lead to known no-regret learning algorithms. Our further experiments demonstrate the effectiveness of our regret-loss, especially in addressing the above ``regrettable'' cases.        
\end{abstract}  


==> conclusion.tex <==
\clearpage
\section{Concluding Remarks}

In this paper, we studied the online decision-making and strategic behaviors of LLMs quantitatively, through the metric of regret. We first examined and validated the no-regret behavior of several representative pre-trained LLMs in benchmark settings of online learning and games. As a consequence, (coarse correlated) equilibrium can oftentimes emerge as the long-term outcome of multiple LLMs playing repeated  games. We then provide some theoretical insights into the no-regret behavior, by connecting pre-trained LLMs to the follow-the-perturbed-leader algorithm in online learning, under certain assumptions.  We also identified (simple) cases where pre-trained LLMs fail to be no-regret, and thus proposed a new unsupervised training loss, \emph{regret-loss}, to provably promote the no-regret behavior of Transformers without the labels of (optimal) actions. We established both experimental and theoretical evidence for the effectiveness of our regret-loss. 

As a first attempt toward rigorously  understanding the online and strategic decision-making behaviors of LLMs through the metric of regret, our work has opened up fruitful  directions for future research: 
\begin{itemize}
    \item There are more than one definitions of (dynamic-)regret in the online learning literature, and we mainly focused on the so-called \emph{external-regret} in the literature. It would be interesting to study the no-regret behavior of LLMs in terms of other regret metrics, e.g., swap-regret \citep{blum2007external}, which may lead to stronger equilibrium notions in playing repeated games. 
    \item  Our new regret-loss has exhibited promises in our experiments for training modest-scale Transformers. We are currently generalizing it to training other larger-scale models, such as Foundation Models, for decision-making. 
    \item No-regret behavior can sometimes lead to better outcomes in terms of social efficiency \citep{blum2008regret,roughgarden2015intrinsic,nekipelov2015econometrics}. It would thus be interesting to further validate the efficiency of no-regret LLM agents in these scenarios, as well as  identifying new prompts and training losses for LLMs to promote the efficiency of the outcomes. 
    \item To evaluate the performance quantitatively, we focused on online learning and games with \emph{numeric valued}  payoffs. It would be interesting to connect our no-regret-based and game-theoretic framework with existing multi-LLM frameworks, e.g., debate, collaborative problem-solving, and human/social behavior simulation, with potentially new notions of regret (defined in different spaces) as performance metrics. 
\end{itemize}









